Device-Free User Authentication, Activity Classification and Tracking using Passive Wi-Fi Sensing: A Deep Learning Based Approach

Privacy issues related to video camera feeds have led to a growing need for suitable alternatives that provide functionalities such as user authentication, activity classification and tracking in a noninvasive manner. Existing infrastructure makes Wi-Fi a possible candidate, yet, utilizing traditional signal processing methods to extract information necessary to fully characterize an event by sensing weak ambient Wi-Fi signals is deemed to be challenging. This paper introduces a novel end to-end deep learning framework that simultaneously predicts the identity, activity and the location of a user to create user profiles similar to the information provided through a video camera. The system is fully autonomous and requires zero user intervention unlike systems that require user-initiated initialization, or a user held transmitting device to facilitate the prediction. The system can also predict the trajectory of the user by predicting the location of a user over consecutive time steps. The performance of the system is evaluated through experiments.

==> relatedwork_rnn.tex <==
Neural networks has been evolving for for decades. People have introduced different neural network architectures for various disciplines. Recurrent Neural Networks(RNN) is the product of derivating the relations between the data samples in a sequence of data. Each RNN unit combines the given input $x_t$, with the previous unit's output $h_{t-1}$ as describe by following $h_t=\psi(W_{hh}h_{t-1}+W_{xh}x_t)$ where $W_{hh}$ and $W_{xh}$ are trainable parameters and $\psi$ is the activation function.

Yet each RNN node does not have access to other data in the sequence except its previous node. Inorder to obtain the information on whole data sequence, Long-Short Term Memory(LSTM)\cite{hochreiter1997long} and Gated Recurrent Unit(GRU)\cite{cho2014learning} were introduced. 
% Due to comparatively low number of parameters and high accuracy, GRU has outperformed the LSTM.\hj{need citation} 

\subsection{Gated Recurrent Units}
GRU cell consists of two gates, update gate $z_t$ and reset gate $r_t$ to regulate the information flow inside the unit. As illustrated in Fig. \ref{fig:gru_cell}, output $h_t$ is an interpolation between previous node activation $h_{t−1}$ and the candidate activation $\Tilde{h_t}$\\
\begin{equation}
    h_t=(1-z_t)+h_{t−1} + z_t \Tilde{h_t}
\end{equation}
where update gate $z_t$ decide by Eq. \ref{eq:update} 
\begin{equation}
   z_t=\sigma(W_zx_t + U_zh_{t−1})
    \label{eq:update}
\end{equation}
and similarly, reset gate $r_t$ is computed using Eq. \ref{eq:reset}
\begin{equation}
   r_t=\sigma(W_rx_t + U_rh_{t−1})
    \label{eq:reset}
\end{equation}
Using $r_t$, candidate activation is calculated using Eq. \ref{eq:cand}
\begin{equation}
   \Tilde{h_t}=tanh(Wx_t + U (r_t \odot h_{t-1}))
    \label{eq:cand}
\end{equation}

\subsection{Bidirectional Gated Recurrent Units}
However, GRU node can acess the data only from it's previous layers. Bidirectional GRU(B-GRU)\cite{graves2013hybrid} allowed a node to access both past and future data by combining a forward GRU and a backward GRU.
BGRU is the step-wise concatenation of the forward
and backward output $h_t:=(\rightarrow h_t ,\leftarrow h_t )$ as shown in Fig. \ref{fig:bigru}
% Traditional B-GRU layer which connects the output of the $l-1^{th}$ layer to the input of the $l+1^{th}$ can be expressed as following layer transition, $x_{l+1}=H_l(x_l)$. Where $x_l$ is the input to the $l^{th}$ layer and $x_{l+1}$ is the input to the ${l+1}^{th}$ layer.

 \begin{figure*} [h]
 \centering
    \subfigure[GRU layer \label{fig:gru}]
    {\includegraphics[scale=0.1]{figures/gru.png}}
    \hspace{1.1cm}
    \subfigure[GRU cell \label{fig:gru_cell}]
    {\includegraphics[scale=0.28]{figures/gru_cell.png}}
    \subfigure[BiGRU layer \label{fig:bigru}]
    {\includegraphics[scale=0.23]{figures/bigru.png}}

\caption{}
\label{fig:system}
\end{figure*}

